On the Asymptotic Performance of Multiple Antenna Channels with Fast Channel Feedback

In this paper, we analyze the asymptotic performance of multiple antenna channels where the transmitter has either perfect or finite bit channel state information. Using the diversity-multiplexing tradeoff to characterize the system performance, we demonstrate that channel feedback can fundamentally change the system behavior. Even one-bit of information can increase the diversity order of the system compared to the system with no transmitter information. In addition, as the amount of channel information at the transmitter increases, the diversity order for each multiplexing gain increases and goes to infinity for perfect transmitter information. The major reason for diversity order gain is a "location-dependent" temporal power control, which adapts the power control strategy based on the average channel conditions of the channel.

==> fig/fig.tex <==

%----------------
% Sec- Problem, fig 1

\begin{figure}[hbtp]
\begin{center}
$\begin{array}{cc}
    \epsfxsize=2in \epsffile{fig/mbyn1} &
    \epsfxsize=2in \epsffile{fig/mbyn2}\\
    \mbox{(a)} & \mbox{(b)}
\end{array}$
\end{center}
\caption{(a) An $M\times N$ channel model, (b) The equivalent channel with $m=\min(M,N)$ parallel channels} \label{fig-mbyn}
\end{figure}

%----------------
% Sec- Feedback, fig 1
\begin{figure}[hbtp]
\centering \epsfysize=2in \epsffile{fig/trunc_step} \caption{An example of a 5-bin channel quantizer with channel inversion
power allocation.} \label{fig-trunc}
\end{figure}

%----------------
% Sec- Feedback, fig 2
\begin{figure}[hbtp]
\centering \epsfysize=2in \epsffile{fig/perf-opt-eq} \caption{Outage for $\log_2(3)$ bits of feedback for optimal, equal
allocation power control, and perfect CSI at Tx and Rx with respect to SNR for a system with single antenna at transmitter and
receiver, and  transmission rate of R=2 b/s/Hz} \label{fig-ossnr}
\end{figure}

